Space-Efficient Data Structures for Polyominoes and Bar Graphs

We provide a compact data structure for representing polyominoes that supports neighborhood and visibility queries. Neighborhood queries concern reporting adjacent cells to a given cell, and visibility queries determine whether a straight line can be drawn within the polyomino that connects two specified cells. For an arbitrary small $\epsilon >0$, our data structure can encode a polyomino with $n$ cells in $(3+\epsilon)n + o(n)$ bits while supporting all queries in constant time. The space complexity can be improved to $3n+o(n)$, while supporting neighborhood queries in $\mathcal{O}(1)$ and visibility queries in $\mathcal{O}(t(n))$ for any arbitrary $t(n) \in \omega(1)$. Previous attempts at enumerating polyominoes have indicated that at least $2.00091n - o(n)$ bits are required to differentiate between distinct polyominoes, which shows our data structure is compact. In addition, we introduce a succinct data structure tailored for bar graphs, a specific subclass of polyominoes resembling histograms. We demonstrate that a bar graph comprising $n$ cells can be encoded using only $n + o(n)$ bits, enabling constant-time query processing. Meanwhile, $n-1$ bits are necessary to represent any bar graph, proving our data structure is succinct.

==> initialSolution.tex <==

We present a compact data structure for storing polyominoes using $3n + o(n)$ bits of space, supporting three types of queries:
\begin{itemize}
\item \emph{neighbourhood queries}: for a cell $c$, report the cell to the left of $c$, $\bm{{\on{left}}}(c)$, the cell to the right of $c$, $\bm{{\on{right}}}(c)$, the cell above $c$, $\bm{{\on{above}}}(c)$, or the cell below $c$, $\bm{{\on{below}}}(c)$.
\item \emph{adjacency queries}: for any two cells $c$ and $c'$, $\bm{{\on{adj}}}(c,c')$ reports whether $c$ and $c'$ are adjacent.
\item \emph{visibility queries}: for any two cells $\cell{x_1}{y_1}$ and $\cell{x_2}{y_2}$, $\bm{{\on{vis}}}(\cell{x_1}{y_1},\cell{x_2}{y_2})$ reports whether $\cell{x_1}{y_1}$ and $\cell{x_2}{y_2}$ are on the same row or column, while the straight line segment from $(x_1,y_1)$ to $(x_2,y_2)$ is contained in $P$.
\end{itemize}
Observe that any data structure that supports navigation queries in time $O(f(n))$ also supports adjacency queries in time $O(f(n))$. In particular, we may answer $\bm{{\on{adj}}}(c,c')$, by checking whether $c' \in \{\bm{{\on{left}}}(c),\bm{{\on{right}}}(c), \bm{{\on{above}}}(c), \bm{{\on{below}}}(c)\}$.

We introduce two solutions; an initial and less involved solution, which supports adjacency, but not navigation and visibility, queries, requiring $4n + o(n)$ bits of space. Moreover, we present a more involved solution that presents a tradeoff between the space requirements, around $3n + o(n)$, and the query time for visibility queries. The latter solution also supports navigation, and thus adjacency, queries in constant time. 

\SubSection{Initial solution}

Given a polyomino $P$, create a breadth-first-traversal tree $T_0$ of $P$ rooted at a cell, $r$.
In $T_0$, we can associate to each node $a$ a label from $\{L, R, T, B\}$ indicating whether $a$ is positioned at the left, right, top, or bottom of its parent's cell (see Figure~\ref{fig:labelled}). Clearly, $T_0$ is sufficient to store $P$. There exist space-efficient data structures for labelled trees of size $n$, where the labels come from an alphabet of size $\sigma$. For example, Geary et al.~\cite{GearyRR06} provide a representation taking $(2+\log \sigma) n +o(n)$ bits of space, supporting a wide range of queries in time $O(1)$. In particular, for any cell $c$ in $P$, and any $\alpha \in \{L,R,T,B\}$, we may query $\bm{{\on{depth}_\alpha}}(c)$ in constant time, reporting the number of ancestors of $c$ that are labelled by $\alpha$.

\begin{figure}
\scalebox{.8}{\figTwoInitSolution}
\centering
\caption{(Left) A polyomino $P$ with numbers corresponding to indices in the breadth-first-traversal of $P$. (Right) the labelled tree $T_0$ associated to $P$.}
\label{fig:labelled}
\end{figure}

\begin{lemma}
The position of a cell, $c$, relative to the root, $r$, can be determined in constant time.
\end{lemma}
\begin{proof}
For each $\alpha \in \{L,R,T,B\}$, query $\bm{{\on{depth}_\alpha}}(c)$. This reveals that on the path from $r$ to $c$ in the breadth-first-traversal, there has been $\bm{{\on{depth}_\alpha}}(c)$ moves in direction $\alpha$. Hence, $c$ is located $\bm{{\on{depth}_T}}(c) - \bm{{\on{depth}_B}}(c)$ cells above and $\bm{{\on{depth}_R}}(c) - \bm{{\on{depth}_L}}(c)$ to the right of $r$ in $P$.
\end{proof}

\begin{theorem}
There exists a data structure that stores polyominoes in $4n + o(n)$ bits of space while supporting adjacency queries in constant time. 
\end{theorem}
\begin{proof}
The space requirement is clear from~\cite{GearyRR06}. For the adjacency queries, pick any two cells $\cell{x_1}{y_1}$ and $\cell{x_2}{y_2}$ in $P$, and determine the relative positions of both $\cell{x_1}{y_1}$ and $\cell{x_2}{y_2}$ to $r$. Then, $\cell{x_1}{y_1}$ is
\begin{align*}
v_d = \bm{{\on{depth}_T}}(\cell{x_1}{y_1}) - \bm{{\on{depth}_B}}(\cell{x_1}{y_1}) - \left(\bm{{\on{depth}_T}}(\cell{x_2}{y_2}) - \bm{{\on{depth}_B}}(\cell{x_2}{y_2})\right)
\end{align*}
cells below $\cell{x_2}{y_2}$, and
\begin{align*}
h_d = \bm{{\on{depth}_R}}(\cell{x_1}{y_1}) - \bm{{\on{depth}_L}}(\cell{x_1}{y_1}) - \left(\bm{{\on{depth}_R}}(\cell{x_2}{y_2}) - \bm{{\on{depth}_L}}(\cell{x_2}{y_2})\right)
\end{align*}
cells to the left of $\cell{x_2}{y_2}$. If $\abs{v_d} + \abs{h_d} = 1$, then $\cell{x_1}{y_1}$ and $\cell{x_2}{y_2}$ are adjacent.
\end{proof}

\begin{example}
Denote by $c_i$ the cell in Figure~\ref{fig:labelled}, which is the $i$'th cell in the breath-first traversal of $P$. Then, to answer $\bm{{\on{adj}}}(c_{13},c_{15})$, we calculate the difference in relative positions of cells $c_{13}$ and $c_{15}$ to the root, $c_0$. 
The path from $c_0$ to $c_{13}$ is $(B, R, B, B, B, L)$ and the path from $c_0$ to $c_{15}$ is $(B, L, B, L, B, B, R)$.
So, 
\begin{align*}
v_d &= (\bm{{\on{depth}_T}}(c_{13}) - \bm{{\on{depth}_B}}(c_{13})) - 
(\bm{{\on{depth}_T}}(c_{15}) - \bm{{\on{depth}_B}}(c_{15})) \\
&= (0 - 4) - (0 - 4) = 0 \\
h_d &= (\bm{{\on{depth}_R}}(c_{13}) - \bm{{\on{depth}_L}}(c_{13})) - 
(\bm{{\on{depth}_R}}(c_{15}) - \bm{{\on{depth}_L}}(c_{15})) \\
&= (1 - 1) - (1 - 2) = 1.
\end{align*}
Since $\abs{v_d} + \abs{h_d} = 1$, we conclude that $c_{13}$ and $c_{15}$ are adjacent. 

To answer $\bm{{\on{adj}}}(c_{13},c_{8})$, we calculate the difference in relative positions of cells $c_{13}$ and $c_{8}$ to $c_0$. 
The path from $c_0$ to $c_{8}$ is $(B, R, B, B)$.
So, 
\begin{align*}
v_d &= (\bm{{\on{depth}_T}}(c_{13}) - \bm{{\on{depth}_B}}(c_{13})) - 
(\bm{{\on{depth}_T}}(c_{8}) - \bm{{\on{depth}_B}}(c_{8})) \\
&= (0 - 4) - (0 - 3) = -1 \\
h_d &= (\bm{{\on{depth}_R}}(c_{13}) - \bm{{\on{depth}_L}}(c_{13})) - 
(\bm{{\on{depth}_R}}(c_{8}) - \bm{{\on{depth}_L}}(c_{8})) \\
&= (1 - 1) - (1 - 0) = -1.
\end{align*}
Since $\abs{v_d} + \abs{h_d} = 2$, we conclude that $c_{13}$ and $c_{8}$ are not adjacent. 
\end{example}


